FoodCHA: Multi-Modal LLM Agent for Fine-Grained Food Analysis

The widespread adoption of camera-equipped mobile devices and wearables has enabled convenient capture of meal images, making food recognition a key component for real time dietary monitoring. However, real-world food images present challenges due to high intra-class similarity and the frequent presence of multiple food items within a single image. While deep learning models achieve strong performance in coarse grained classification, they often struggle to capture fine-grained attributes such as cooking style. Moreover, open-ended generation in modern vision-language models can produce non-canonical labels, limiting their practical deployment. We propose FoodCHA, a multimodal agentic framework that reformulates food recognition as a hierarchical decision-making process. By progressively anchoring predictions, FoodCHA guides subcategory identification using high-level categories and guides cooking style recognition using subcategories, improving semantic consistency and attribute-level discrimination. To ensure practical deployability, FoodCHA utilizes the compact Moondream-2B vision language model, which provides strong reasoning capability while maintaining lower computational and memory overhead. Experiments on FoodNExTDB show that FoodCHA outperforms Food-Llama-3.2-11B by 13.8% and 38.2% in category and subcategory recognition precision, respectively, and achieves a striking 153.2% improvement in cooking style classification precision.

==> relteadworkV1.tex <==
\section{Related works}
\subsection{Food Recognition based on Deep Learning Network} 
Food recognition tasks has been widely studied using deep learning architectures such as models that are based on Convolutional Neural Networks. To help us with our work with FoodCHA we felt it was important to look at these type of models as a baseline for our experiments.
\subsubsection{CNN Baselines}
    CNNs such as ResNet have been the dominant backbone for food recognition tasks. These models leverage deep residual layer connections to extract visual features. While ResNet achieves very solid performance in food category classification, it doesn't perform nearly as well for more detailed and nuanced tasks such as subcategory and cooking style classification. Extensions like Squeeze-and-Excitation Networks (SENet) and SGLANet further improve how the model is able to identify subtleties within images [1]. Even though these CNN variants improved accuracy on datasets such as Food101, their performance generally fell short of expectations when applied to more complex datasets such as FoodNExTDB. 
\subsubsection{NoisyViT}
    We then looked to Vision Transformer (ViTs) models as a possible capable alternative. ViTs model long-range dependencies between ingredients and plating arrangements[2]. However, standard ViTs overfit and are sensitive to real-world image noise. NoisyViT addresses these limitations by injecting structured noise into attention layers[2]. In doing so, the model reduces task complexity, improves generalization, and improves robustness of the model against visual variations in the images. The experiments show that NoisyViT outperforms the traditional CNN baselines we tried before. This highlights NoisyViT;s effectiveness in fine-grained food recognition and its potential for dietary assessment in healthcare applications. On the other hand, this approach still doesn't perform as well as existing state of the art models like Chat-GPT, Gemeni, and Claude when it comes to performance.
\subsubsection{CVNet}
    In parallel, we also looked at the CVNet light CNN-transformer hybrid architectures that balance efficiency and accuracy. Lee et al. propose CVNet, a learned re-ranking method for instance-level image retrieval that replaces classical geometric verification with correlation verification [3]. In a food recognition context, CVNet can use its retrieval based pipelines for food understanding by retrieving visually similar dishes from a labeled gallery, which can help with fine-grained and long tail categories. However, this differs fundamentally from our approach. FoodCHA is a dataset constrained, hierarchical prediction system (category → subcategory → cooking style) that uses priors and normalization to produce canonical labels directly from a single image, whereas CVNet focuses on pairwise similarity re ranking and requires a reference database rather than producing structured, multi-attribute outputs.


\subsection{Food Recognition based on Large Language Model} 
\subsubsection{FoodLLM}
Regarding food recognition using LLMS/VLMs, other proposed solutions have included multi-modal models such as FoodLLM by Yin et al. This food assistant aims to combine food classification, ingredient recognition, recipe generation, nutrition estimation, referring segmentation, and reasoning segmentation through a base LLAMA LLM model and a SAM segmentation model[5]. It utilizes five datasets in a two-stage training process to fine-tune and advance its abilities in multi-round conversations with users. Our goal and efforts differ as it is more focused on accurate food recognition, relying on the FoodNExtDB dataset to train and finetune various LLMs and VLMs to categorize foods into categories, subcategories, and cooking/preparation styles. This, while creating a simpler training stage, allows us to gain further breadth and perspective on the state and real-world efficacy of LLMs and VLMs for food recognition today. 
\subsubsection{ResV-Mamba}
Selective state space models (SSMs) have recently emerged as a strong alternative to attention-based ViTs for visual recognition. An example of this has been applied to fine-grained food classification via VMamba. Chen et al. propose Res-VMamba, which augments VMamba’s multi-stage visual state space backbone with a global residual design to better combine global context and local discriminative cues[4]. They evaluate on CNFOOD-241 and report that VMamba-based models outperform several CNN/ViT baselines under their proposed split. This differs from our FoodCHA approach because ResV-Mamba improves the backbone used for food classification, while FoodCHA changes the inference paradigm, turning open-ended VLM outputs into controlled, hierarchical decisions aligned to a fixed label space.
\subsubsection{FoodSky}
Another domain specific LLM we looked at was FoodSky. Zhou et al. introduce FoodSky, a food-oriented large language model designed to answer culinary and dietetic questions at an expert level [6]. Their main premise is that general-purpose LLMs often lack depth and reliability in food and nutrition topics, so FoodSky is trained on a large, curated food corpus (FoodEarth) assembled from authoritative sources.In evaluation, FoodSky shows strong performance on food-domain benchmarks and notably achieves high accuracy on Chinese chef and dietetic examinations, demonstrating the value of building a specialized foundation model for food knowledge and dietary guidance. This differs from our work because FoodSky primarily targets text-based food knowledge, reasoning, and question answering, whereas our work targets vision-based food recognition in real images with structured, dataset-constrained outputs.

